Paradigm Shift in Infrastructure Inspection Technology: Leveraging High-performance Imaging and Advanced AI Analytics to Inspect Road Infrastructure

Effective road infrastructure management is crucial for modern society. Traditional manual inspection techniques remain constrained by cost, efficiency, and scalability, while camera and laser imaging methods fail to capture subsurface defects critical for long-term structural integrity. This paper introduces ROVAI, an end-to-end framework that integrates high-resolution X-ray computed tomography imaging and advanced AI-driven analytics, aiming to transform road infrastructure inspection technologies. By leveraging the computational power of world-leading supercomputers, Fugaku and Frontier, and SoTA synchrotron facility (Spring-8), ROVAI enables scalable and high-throughput processing of massive 3D tomographic datasets. Our approach overcomes key challenges, such as the high memory requirements of vision models, the lack of labeled training data, and storage I/O bottlenecks. This seamless integration of imaging and AI analytics facilitates automated defect detection, material composition analysis, and lifespan prediction. Experimental results demonstrate the effectiveness of ROVAI in real-world scenarios, setting a new standard for intelligent, data-driven infrastructure management.

==> algorithms/block.tex <==
\begin{figure}[t]
\begin{algorithm}[H]
\flushright
\begin{minipage}{0.95\linewidth}
\caption{Offset-scan Back-projection algorithm layout before and after optimization. 
}
\label{alg:BPOpt}
\small
\LinesNumbered
\KwIn{Before optimization $input[N_v][N_r][N_c]$ projections.}
\KwOut{Before optimization $output[N_z][N_y][N_x]$ volume.}

{
% \normalem

\For{$y=0$ \textbf{to} $N_y$}{

    \For{$x=0$ \textbf{to} $N_x$}{

        \For{$z=0$ \textbf{to} $N_z$}{
        
            val = 0.0; \Comment{\textcolor{blue}{//Scalar}}
            
            \For{$v=0$ \textbf{to} $N_v$}{
            
                $\mathrm{i_{det}}$ = Proj(x, y, v);
                
                val += input[v][z][$\mathrm{i_{det}}$]; \Comment{\textcolor{blue}{//Scalar}}
                
            }
            output[z][y][x] = val; \Comment{\textcolor{blue}{//Scalar}}

        }
    }
}
}

\KwIn{After optimization $input[N_c][N_v][N_r]$ projections.}
\KwOut{After optimization $output[N_y][N_x][N_z]$ volume.}

{
% \normalem
    
\For{$yy=0$ \textbf{to} $N_y$ \textbf{step} $N_{y\_block}$}{

    \For{$xx=0$ \textbf{to} $N_x$ \textbf{step} $N_{x\_block}$}{
    
        \For{$y=0$ \textbf{to} $N_{y\_block}$}{
        
            \For{$x=0$ \textbf{to} $N_{x\_block}$}{

                $\mathrm{y_{det}}$ = yy * $N_{y\_block}$ + y; 
                
                $\mathrm{x_{det}}$ = xx * $N_{x\_block}$ + x;
        
        \For{$z=0$ \textbf{to} $N_z$}{

            val[z] = 0.0; \Comment{\textcolor{blue}{//Vector}}
        }
        
        \For{$v=0$ \textbf{to} $N_v$}{

            $\mathrm{i_{det}}$ = Proj($\mathrm{x_{det}}$ $\mathrm{y_{det}}$, v);

            \For{$z=0$ \textbf{to} $N_z$}{
                
                val[z] += input[$\mathrm{i_{det}}$][v][z]; \Comment{\textcolor{blue}{//Vector}}
                
            }
        }
        
        \For{$z=0$ \textbf{to} $N_z$}{
        
            output[$\mathrm{y_{det}}$][$\mathrm{x_{det}}$][z] = val[z]; \Comment{\textcolor{blue}{//Vector}}
            
        }
        }
        }

        }
    }
}
}

\end{minipage}
\end{algorithm}

\end{figure}

==> tables/param.tex <==

%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]  
\centering
\caption{ 
Parameters used in ROVAI. The upper section lists acquisition-specific parameters, the lower section defines parallelization settings.}        
    \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1.08}% Tighter
        \begin{tabular}{ ?c|l? }
        \tbhline
        \bf{Symbol} & \bf{Description} \\
        \hline
        $N_{specimen}$  & Number of specimens \\
        $N_p^i$ & Number of projection angles in $i^{\text{th}}$ specimen (K in Eqn~\ref{eqn:bp}) \\
        $N_c^i$ & Detector channels of the 2D projection in $i^{\text{th}}$ specimen  \\
        $N_r^i$ & Detector rows of the 2D projection in $i^{\text{th}}$ specimen \\
        $N_x^i, N_y^i, N_z^i$ & Dimensions of 3D volume in the X, Y, and Z in $i^{\text{th}}$ volume \\
        % $Model_{AI}$ & AI inference model \\
        % $V_{SAP}$ & Volume slice patches after the SAP process \\
        \hline
        $P_{row}$ & Number of row parallel MPI nodes \\
        $P_{proj}$ & Number of projection parallel MPI nodes \\
        $P_{slice}$ & Number of slice parallel MPI nodes \\
        $\mathbb{G}$ & Set of group row partitions\\
        $\mathbb{P}$ & Set of hyperparameters: $P_{row}$, $P_{proj}$, $P_{silce}$, and $\mathbb{G}$ \\
        \hline
        \tbhline
        \end{tabular}
        }
\label{tab:param}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]  
% \centering
% \caption{ 
% Parameters used in ROVAI. The top section lists acquisition-specific parameters, the middle section defines parallelization settings, and the bottom section includes system-level parameters specific to the Fugaku.}        
%     \resizebox{\linewidth}{!}{
%     %\renewcommand{\arraystretch}{1}% Tighter
%         \begin{tabular}{ ?c|l? }
%         \tbhline
%         \bf{Symbol} & \bf{Description} \\
%         \hline
%         $N_{specimen}$  & Number of specimens \\
%         $N_p^i$ & Number of projection angles in $i^{\text{th}}$ specimen (K in Eqn~\ref{eqn:bp}) \\
%         $N_c^i$ & Detector channels of the 2D projection in $i^{\text{th}}$ specimen  \\
%         $N_r^i$ & Detector rows of the 2D projection in $i^{\text{th}}$ specimen \\
%         $N_x^i, N_y^i, N_z^i$ & Dimensions of 3D volume in the X, Y, and Z in $i^{\text{th}}$ volume \\
%         $Model_{AI}$ & AI inference model \\
%         $V_{SAP}$ & Volume slice patches after the SAP process \\
%         \hline
%         $P_{row}$ & Number of row parallel MPI nodes \\
%         $P_{proj}$ & Number of projection parallel MPI nodes \\
%         $P_{slice}$ & Number of slice parallel MPI nodes \\
%         $\mathbb{G}$ & Set of group row partitions\\
%         $\mathbb{P}$ & Set of hyperparameters: $P_{row}$, $P_{proj}$, $P_{silce}$, and $\mathbb{G}$ \\
%         \hline
%         $BW_{2ndS}$  & Bandwidth of the Fujitsu Exabyte File System~\cite{FEFSGuide} \\
%         $BW_{1stS}$  & Bandwidth of the Lightweight Layered IO-Accelerator~\cite{LLIOGuide} \\
%         % $BW_{M}$ & Bandwidth of local memory \\
%         $TH^{P}_{reduce}$ & Throughput of \textsf{MPI\_Reduce\_scatter\_block} on $P$ nodes \\
%         $TH^{P}_{alltoall}$ & Throughput of \textsf{MPI\_Alltoallv} on $P$  nodes \\
%         $TH^{P}_{bcast}$ & Throughput of \textsf{MPI\_Bcast} on $P$ nodes \\
%         $CC_{BP}$ & Computational capability for back-projection \\
%         $CC_{AI}$ & Computational capability for AI inference \\
%         $CC_{other}$ & Computational capability for other tasks (e.g., FFT, SAP) \\
%         \tbhline
%         \end{tabular}
%         }
% \label{tab:param}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
\newcommand{\tbhline}{\noalign{\hrule height 1pt}}
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.15}
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}[t]  
 \centering
  \caption{The parameters for the ROVAI framework. The upper parameters affect the computation amount of the overall problem, the middle parameters are the hyper-parameters that define the parallelization of our framework, and the lower are acquisition measurement configuration parameters.}        
      
      \resizebox{\linewidth}{!}
      {
      \renewcommand{\arraystretch}{0.95}% Tighter
      \begin{tabular}{ ?c|c|l? }
      \tbhline
      & \bf{Symbol} & \bf{Description}\\
      \hline
      \multirow{5}{*}{\rotatebox[origin=c]{90}{Definition}} & $N_{sub\_scan}$  & Number of total sub-scans,  \\
      & $N_v^i$      & Number of projection views, \chen{corresponding to \( K \) in Eqn~\ref{eqn:bp}} \\
      & $N_r^i, N_c^i$ & Rows and Channels of 2D projection in $i^{th}$ sub-scan \\
      & $N_x^i, N_y^i, N_z^i$ & Dimension of 3D volume in X, Y, Z-axis in $i^{th}$ sub-scan \\
      & $Model_{AI}$ & The AI inference  model\\
      & $V_{SAP}$ & The volume patches after SAP process\\
      \hline
      \multirow{5}{*}{\rotatebox{90}{\makecell{Hyper}}} & $P_{sub\_scan}$ & Number of sub-scan partitioning \\
      & $P_{proj}$ & Number of projection partitioning \\
      & $P_{vol}$ & Number of volume partitioning \\
      & $\mathbb{G}$ & A set of group sub-scans after partitioning \\
      & $\mathbb{P}$ & A set of hyper-parameters $P_{sub\_scan}$, $P_{proj}$, $P_{vol}$, and $\mathbb{G}$ \\
      \hline
      \multirow{8}{*}{\rotatebox{90}{\makecell{Measurement}}} & $BW_{2ndS}$  & Bandwidth of Fujitsu Exabyte File System~\cite{FEFSGuide} \\
      & $BW_{1stS}$  & Bandwidth of Lightweight Layered IO-Accelerator~\cite{LLIOGuide}\\
      & $BW_{M}$ & Bandwidth in local memory\\
      & $TH^{P}_{reduce}$ & Throughput of MPI\_Reduce\_scatter\_block in P nodes \\
      & $TH^{P}_{alltoall}$ & Throughput of MPI\_Alltoallv in P nodes\\
      & $TH^{P}_{bcast}$ & Throughput of MPI\_Bcast in P nodes\\
      & $CC_{BP}$ & Computational capability of Back-Projection \\
      & $CC_{AI}$ & Computational capability of AI Inference \\
      & $CC_{other}$ & Computational capability of other (e.g. FFT, SAP) \\
      \tbhline
      \end{tabular}  
      }

    %\begin{tablenotes}
    %    \footnotesize
    %    \raggedright
    %    \item *1. FEFS: Fujitsu Exabyte File System\cite{akimoto2020file,FEFSGuide}.
    %    \item *2. LLIO: Lightweight Layered IO-Accelerator\cite{akimoto2020file,LLIOGuide}.
    %\end{tablenotes}
\label{tab:param} 

\end{table}     
%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}



==> tex.sc25/0_keywords.tex <==
\keywords{
Imaging, AI, HPC, Road Inspection
}


==> tex.sc25/0_title.tex <==
%An End-to-end Imaging and Analysis Framework using Supercomputing and AI
%\title{Paradigm Shift in Infrastructure Inspection Technology}     

%\title{\fontsize{24pt} Paradigm Shift in Infrastructure Inspection Technology}
\title{{\fontsize{23pt}{26pt}\selectfont Paradigm Shift in Infrastructure Inspection Technology}

\thanks{$\dagger$ Co-first authors}
}


%\title{Paradigm Shift in Infrastructure Inspection Technology: \\ \LARGE  Leveraging High-performance Imaging and Advanced AI Analytics to Inspect Road Infrastructure}     

==> tex.sc25/3_overview.tex <==

\input{tables/road_inspection}
% \section{Overview of \textit{ROVAI}}
Fig.~\ref{fig:overview} presents an overview of \textit{ROVAI}. Dozens of specimens have been collected, and collection will continue, from the national highway network e.g. from the Kansai urban region of western Japan. This area is home to over 20 million people, with major cities including Osaka, Kyoto, and Kobe. The highway network spans more than 250 km and carries approximately 700,000 vehicles per day. Since over 2/3 of the network is more than 30 years old, it is essential to develop effective technologies to identify road segments that are prone to critical failures. These include delamination, cohesive failure, insufficient asphalt coverage around aggregates, and cracking of the aggregates themselves. The specimens are transported to SPring-8, a leading synchrotron radiation facility, where they are scanned in high resolution XCT. The scans were then moved to the Fugaku supercomputer facility, at which a high throughput image reconstruction pipeline we developed was used to reconstruct the 3D images of dozens of specimens with 10,000s of compute nodes. While Fugaku is a capable supercomputer, its processors lack matrix processing units and support for lower precision. To that end, effective training of a foundation model was done on a supercomputer more suitable for the task. The 3D images reconstructed on Fugaku were then moved to Frontier supercomputer to train a vision transformer foundation model for 3D volumetric segmentation on 1,000s of GPUs. The foundation model include key innovations such as a simulator for generating masks and symmetric adaptive patching. Next, the model was fine-tuned, and the model weights were moved to Fugaku supercomputer. Finally, we conducted full scale Fugaku runs to demonstrate, at full system capacity, the ability to simultaneously reconstruct dozens followed by AI inference, in a single fused end-to-end pipeline: from loading the scans from the PFS I/O to writing back the 3D segmented images to storage. 

The framework, \textit{ROVAI}, is intended for ongoing future use on new specimens that would be regularly collected, positioned to be a paradigm shift in infrastructure inspection. Table~\ref{tab:road_inspection} overviews the key inspection tasks that \textit{ROVAI} can enable. First, detecting the early formation of cracks. Second, monitoring the evolution of crack shapes over time to gain insights into their growth patterns and potential failure points. Third, analyzing the particle size distribution of aggregates, such as gravel and air pockets, in specific regions helps assess material consistency and identify anomalies that could affect durability. Finally, future additional AI-driven analytical capability have the potential to allow for precise deterioration predictions by assessing long-term environmental impacts, enabling proactive maintenance strategies. 

%Fig.~\ref{fig:overview} gives a general overview of \textit{ROVAI}. Dozens of specimens were collected, and will continue to be collected, form the national highway network in the Kansai urban region in west Japan, which has a population of over 20M people concentrated in large cities such as Osaka, Kyoto, Kobe etc. The national highway network spanning the region has a total distance of over 250KM with a traffic volume of 700K cars per day. With more than 2/3 of the highways in the network being above 30 years old, it is crucial to find effective technologies for identify road segments prone to different types of critical failures: delamination, cohesive failure, lack of asphalt coverage around aggregates, and cracking of the aggregate itself. The asphalt core specimens are delivered to SPring-8, a flagship synchrotron facility, at which they are scanned. 




\begin{comment}
\wahib{The following is the list of key requirements needed to assess the condition of infrastructure asphalt and concrete specimens:
a) finding of initiation of cracks in 3D models, b) tracking of the shape changes of crack initiation, c) particle size distribution of aggregates in specified areas, and d) deterioration prediction by CTs of accelerated degradation.}
\end{comment}



==> tex.sc25/5_AI_training.tex <==



\section{Foundation Model for High-resolution 3D Segmentation}\label{sec:AI_training}
The core requirement from an AI vision model that can enable the analytics required for robust inspection of road infrastructure is high-quality 3D volumetric segmentation. Building downstream functionalities become straightforward, once high-quality segmentation exists. High-quality segmentation is a challenging problem, for three reasons. First, high quality datasets are necessary. Second, labeling large datasets of high-resolution 3D volumes is unfeasible. Third, the memory requirements for high-resolution segmentation are notoriously restrictive. In this section we discuss the design and training process of the vision transformer foundation model we developed for this project. Note that the model, that we openly release, can be used stand-alone for segmentation of high-resolution concrete, asphalt, sand etc 3D images. 

\begin{comment}    
{\color{red} Copy from introduction} 
\textit{Training segmentation model on our real-world road concrete and asphalt composites dataset}: There is no prior work on training transformer-based model in a label-free manner on such high-resolution CT images. The common ViT~\cite{dosovitskiy2020image} method converts high-resolution images into patches as input for training a transformer-based model, resulting in an ultra-long sequence length~\cite{zhang2024adaptive}. With a sequence length-to-model size relationship of $O(n^2)$, excessively long sequences can make the model computationally expensive and memory-intensive, making training impractical~\cite{wang2023ultra}. Another challenge in training model is that training requires labels. Since our dataset comes from the real-world and it is not realistic to annotate such high-resolution CT image pixel by pixel, the generation of labels is difficult. To that end, we leverage multiple advanced AI models and techniques, including SAM 2~\cite{ravi2024sam}, Generative Adversarial Network(GAN)~\cite{ziabari2021high,akkem2024comprehensive}, Masked Auto Encode(MAE)~\cite{he2022masked}, Symmetrical Adaptive Patching(SAP)~\cite{zhang2024adaptive}, to train the segmentation model on our real-world dataset.
\end{comment}

\subsection{Generating Labeled Data by Simulating Reconstruction}
\label{sec:sim}
To generate training data for the model, we simulated high-resolution synchrotron CT data of concrete by developing a scalable pipeline that transforms large-scale virtual microstructures into realistic XCT scan volumes. 
Starting from volumetric data generated using PyCMG~\cite{PyCMG} at a coarse resolution of 150 $\mu m$, the pipeline extracts multiple sub-volumes and resamples them to a resolution of 12.02 µm, matching the voxel size of real synchrotron CT scans. 
Each resampled sub-volume is randomly cropped along the z-axis to a depth between 50 and 120 slices, resulting in 3D volumes of approximately $8192 \times 8192$  pixels per slice. 
These high-resolution volumes are then passed through an XCT forward model using the ASTRA toolbox~\cite{van2016fast} with an FBP reconstruction algorithm, simulating realistic XCT projections and reconstructions. 
Material-specific attenuation coefficients—derived from regions of interest in real synchrotron scans of pores, cement paste, aggregates, and background—are used to assign physically meaningful intensities. 
Each volume is further processed under varying conditions, including multiple projection sparsity levels, applying Poisson and adding Gaussian noise, Gaussian blurring in the projection data, and synthetic ring artifacts to replicate common experimental degradations. 
In total, 780 unique volumes were generated, providing a diverse dataset for robust machine learning training. This comprehensive synthetic dataset serves as a valuable resource for downstream fine-tuning tasks such as segmentation as well as reconstruction, and representation learning. 
%In future work, we plan to enhance this pipeline using constrained CutGAN to generate even more realistic augmentations of real synchrotron concrete scans.

\subsection{Self-Supervised Learning with MAE}
\label{sec:mae}

Training accurate segmentation models that generalize well requires large labeled datasets, but generating such data is time-consuming and biased. In our case, obtaining large labeled datasets is unfeasible, though we have access to substantial unlabeled data. To address this, we leverage unsupervised learning to pre-train models, capturing broad features for downstream tasks.
Transfer learning is a common approach in AI/ML, where features from pre-trained models are adapted to new tasks. ViTs, in particular, excel in transfer learning. We utilize pre-trained ViT models, such as SAM 2~\cite{ravi2024sam2}, for segmentation. However, these models are trained on significantly different data from our high-resolution 3D datasets, prompting us to explore self-supervised pre-training with a Masked Autoencoder (MAE).

Self-supervised pre-training enables large-scale ViT training using our vast data resources, producing versatile models for various segmentation tasks, including simulated labeled data. The initial MAE models, following the ViT-Base size, serve as proofs of concept. Scaling them further is feasible, and we plan to explore parallelism techniques from the 2024 Gordon Bell Finalist ORBIT~\cite{10793137} to enhance downstream segmentation performance. Importantly, these models must efficiently perform inference within the image reconstruction pipeline to compute in situ metrics.

\begin{comment}
Training highly accurate segmentation models that also generalize well over a wide distribution of data requires access to large amounts of labeled datasets. We can create simulated labeled data from the processes described in the previous section, which can provide an invaluable tool to aid in fine-tuning segmentation models for the eventual segmentation of human-labeled data. However, this process is also limited due to the manual and time-consuming process required to generate the data along with the biases in the choices made when generating the data. Ultimately, this limits the amount and generalizability of the training data.

In our case, it is unfeasible to obtain the large labeled datasets needed to create the large generalizable segmentation models desired; however, we do have access to a large amount of unlabeled data. Therefore, we can use alternative strategies via unsupervised learning methods to pre-train models to capture features from across the data, which can then be used as a launching point for downstream tasks.

In the case of limited labeled data, it is common practice across the field of AI/ML  to take advantage of the transfer learning capabilities from the so-called pre-trained models to transfer the features those models have learned to other models. ViT's in particular have been shown to perform well in the area of transfer learning. In essence, this transfer learning process includes extracting the model weights from a ViT's encoder and fine-tuning those weights along with a specialized decoder for a specific downstream task.


There are a variety of different publicly available pre-trained ViT models that have been trained across a multitude of different datasets and tasks. In the following section, we demonstrate the use of one such pre-trained model, SAM (a ViT model trained for segmentation), to fine-tune a segmentation model for our data. However, the issue with using pre-trained models is that they are trained on data far different from the high-resolution 3D data in our work. For instance, the images SAM is trained on are 3300×4950 pixels on average, and also have different features than our data. Therefore, we investigate pre-training our own ViT models via a self-supervised Masked Autoencoder (MAE) model to show the benefits.

The ability to pre-train models on a self-supervised task opens the door to training large-scale ViT models due to the vast amount of data we have access to. Once trained to learn across a wide distribution of data, the pre-trained model can then be used as an all-purpose model for all varieties of downstream fine-tuning datasets and tasks that are developed for the data, including the simulated labeled data. The benefit of doing the upfront computations to pre-train a large specialized MAE model then lies in the decreased training required for the different downstream fine-tuning tasks. 

Due to the nature of the high-resolution data, the MAE pre-training that we perform employs the adaptive patching technique used in the SAP method described in the following section. The MAE models that we initially train are relatively small in terms of model size following the ViT-Base size, but serve as a proof of concept of the methodology along with the fine-tuned counterparts in the following section. The size of MAE models we can scale to is very large given the amount of data we have available. We plan to investigate the utility of scaling these models using parallelism techniques from 2024 Gordon Bell Finalist ORBIT [CITE] and show how reasonable and effective it is to use these larger models to improve performance on the downstream segmentation task. However, it must be noted that the purpose of these models is to use within the image reconstruction pipeline to calculate in situ metrics and thus it is important to provide a model that can efficiently perform inferencing within that pipeline.
\end{comment}

\subsection{Symmetric Adaptive Patching}\label{sec:SAP}

\textbf{Base Model:} We use the well-known segmentation model SAM 2 \cite{kirillov2023segment}, its encoder to be specific, as a base model that we adapt. SAM 2 employs a ViT encoder as its backbone for segmentation tasks. SAM 2 offers ViT variants (ViT-Base (b), ViT-Large (l), and ViT-Huge (h)), each with 12, 24, or 32 transformer layers, respectively. These weight configurations—b, l, and h—are pre-trained using Masked Autoencoders (MAE) \cite{he2022masked}. 
%Unlike Unet-style models \cite{ronneberger2015u, hatamizadeh2022unetr, cao2022swin}, SAM 2’s mask decoder is lightweight, containing only two convolutional layers. However, reconstructing high-resolution masks from the latent space requires additional upscaling layers, leading to increased memory usage. 

\textbf{Symmetrical Adaptive Patching (SAP):} SAP is a method for hierarchical image segmentation that enhances model learning by extracting multiscale spatial structures from input images. SAP takes inspiration from the use of adaptive patching in 2D pathology images~\cite{zhang2024adaptive}. The key stages are as follows:
(1) Edge Detection:
Uses Canny edge detection~\cite{canny1986computational}, and the final results are robust to threshold-value variations. This process extracts hierarchical details as grayscale edges, smoothing out irrelevant features while preserving structural information.
%Uses Canny edge detection [CITE] (note that final result are robust to random thresholds) to extract hierarchical details, producing grayscale edges. Smooths irrelevant details while preserving structural information.
(2) Adaptive Patches: AP first constructs quadtrees (2D) or octrees (3D) by recursively partitioning edge-detected images. To construct the tree $L$, AP creates tree nodes $L_n$ representing specific regions where $n$ is the number of the leaf nodes. The leaf nodes $L_{n+s-1}$ is defined recursively as follows:
\begin{equation}\begin{aligned}\footnotesize
L_{n+s-1} = \begin{cases} 
L_n, & \text{if $n \geq N$} \\
L_n[i] = \{L^{\text{1}}_n, L^{\text{2}}_n, ..., L^{\text{s}}_n\}, & \text{$\arg\max\limits_i V(L_n[i])$}
\end{cases}
\end{aligned}\end{equation}
where $V$ is the criterion we use to differentiate the different levels of details. We choose the maximum sum of pixel values among the tree nodes as $i = \arg\max\limits_i V(L^n[i])$.
%\begin{equation*}\footnotesize
%\begin{aligned}
%    i = \arg\max\limits_i V(T^n[i])
%\end{aligned}
%\end{equation*}
%$ i = \arg\max\limits_i V(T^n[i])$, 
The set $\{L^{\text{1}}_n, L^{\text{2}}_n, ..., L^{\text{s}}_n\}$ represents the $s = 2^d$ new child nodes created after subdividing $L^n[i]$, where $d$ is the number of dimensions. For example, $s = 4$ and $s = 8$ correspond to quadtree and octree structures, respectively~\cite{samet1984quadtree, finkel1974quad}.
Then, splits regions based on pixel intensity variance, ensuring uniform sequence length for GPU efficiency. Finally, generates patch sequences via Z-order space-filling curves, maintaining alignment between image and mask patches.
(3) Depatching: Reconstructs masks during inference by upscaling patch sequences using the original quad/octree structure. Eliminates the need for U-Net decoders by using sparse mask information.

\subsection{Training Our Foundation Model}
In Fig.~\ref{fig:AI_overview}, we present the complete training flow of our foundation model. We trained the model in two steps. First, we perform pre-training on label-free high-resolution images using MAE (as described in Section~\ref{sec:mae}). The pre-training phase uses 45 sample groups, with each group trained for a total of 800 epochs. The training is conducted on 2,048 GPUs provided by Frontier. Through MAE pre-training, we enhance the model’s generalization capability on real-world data.

Next is the fine-tuning stage. We first employ the simulated reconstructed method we introduced in Section~\ref{sec:sim} to generate high-precision data and labels, totaling $62,400$ $8K^2$ 2D slices ($780\times80$). We then replace the ImageEncoder in SAM 2 with the pre-trained MAE weights and split the synthetic dataset into training and testing sets at a $85\!:\!15$ ratio for fine-tuning. Additionally, to address the long-sequence issue inherent in attention mechanisms, we adopt SAP to reduce computational overhead. The Evaluation section provides quantitative and qualitative comparisons between our model and baselines.

==> tex.sc25/6_end2end_optimization.tex <==

\section{Fusion of Image Reconstruction and AI inference in to a Single Pipeline}\label{sec:end2end}
%\section{Collaborative End-to-end Scaling and Pipeline Optimization}\label{sec:end2end}
This section focuses on optimizing the image reconstruction and AI-driven analysis pipeline to eliminate redundant I/O operations. Our goal is to minimize unnecessary data transfers and enhance overall efficiency. 
% We quantitatively analyze the performance gain resulting from this optimization, emphasizing its effects on throughput, latency, and resource utilization.

%We focus on eliminating redundant PFS I/O operations by designing an efficient image reconstrucion and AI-driven analysis pipeline. We quatatively analysze the benefits of building the pipeline.
%efficiently merging image reconstruction with AI segmentation workflows with minimal overhead. First, we assess how I/O bottlenecks impact framework performance and why optimization is essential. Next, we introduce how to coordinate the scaling between image reconstruction and AI-driven segmentation. And we integrate these two components distributed into a unified pipeline to enhance the end-to-end efficiency of our ROVAI framework without losing scalability.


\begin{figure}[t]
\begin{center}

\begin{minipage}{0.485\textwidth}
    \includegraphics[clip,width=1\textwidth]{figures/merge_AI.pdf}
    \caption{
    %Workflow for merging distributed image reconstruction with AI segmentation.
    Memory-resident end-to-end pipeline for distributed image reconstruction fused with 3D segmentation.
    }
    \label{fig:merge_AI}
\end{minipage}

\vskip 5pt

\begin{minipage}{0.485\textwidth}
    \includegraphics[clip,width=1\textwidth]{figures/pipeline_comp.pdf}
    \caption{Pipeline optimization runtime measured in seconds. (a) is the step-wise workflow aligned with different stages of our performance model. The dotted box highlights a detailed view of two computation stages. (b) Example pipeline for H\textsuperscript{3} imaging using optimal scaling strategies (P\textsubscript{proj}=48, P\textsubscript{slice}=16, $\lvert \mathbb{G} \rvert$=8) across 12,288 nodes. (c) Example pipeline for entire ROVAI framework using optimal scaling strategies (P\textsubscript{proj}=48, P\textsubscript{slice}=4, $\lvert \mathbb{G} \rvert$=16) across full Fugaku: 152,064 nodes.}
    \label{fig:pipeline}
\end{minipage}

\end{center}
\end{figure}


% %%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%   \begin{center}
% \includegraphics[clip,width=0.49\textwidth]{figures/merge_AI.pdf}
%     \caption{
%     %Workflow for merging distributed image reconstruction with AI segmentation.
%     Memory-resident end-to-end pipeline for distributed image reconstruction fused with 3D segmentation.
%     }
%     \label{fig:merge_AI}
%   \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%   \begin{center}
% \includegraphics[clip,width=0.49\textwidth]{figures/pipeline_comp.pdf}
%     \caption{Pipeline optimization runtime measured in seconds. (a) is the step-wise workflow aligned with different stages of our performance model. The dotted box highlights a detailed view of two computation stages. (b) Example pipeline for H\textsuperscript{3} imaging using optimal scaling strategies (P\textsubscript{proj}=48, P\textsubscript{slice}=16, $\lvert \mathbb{G} \rvert$=8) across 12,288 nodes. (c) Example pipeline for entire ROVAI framework using optimal scaling strategies (P\textsubscript{proj}=48, P\textsubscript{slice}=4, $\lvert \mathbb{G} \rvert$=16) across full Fugaku: 152,064 nodes.}
%     \label{fig:pipeline}
%   \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%

\subsection{Memory-resident End-to-end Pipeline}\label{sec:workround_storage}
To mitigate performance bottlenecks caused by frequent I/O operations on the PFS, \emph{ROVAI} implements a memory-resident end-to-end pipeline, as shown in Fig.~\ref{fig:merge_AI}. In this design, high-resolution 3D volumetric data (more than 2TB per volume), generated by the FPB module, is stored entirely in system (or host) memory. This allows downstream AI tasks, like semantic segmentation, to directly access the data without having to load or store it from the PFS, eliminating redundant I/O operations.
By keeping the data in memory throughout the pipeline, \emph{ROVAI} reduces pipeline stalls, prevents unnecessary data transfers, and improves processing efficiency. This is particularly important for \emph{ROVAI}, where the PFS I/O can be a significant bottleneck when performing full-system scale parallel computing for FBP image reconstruction and AI-driven 3D image analysis.
%This approach also minimizes reliance on the PFS, alleviates bandwidth contention, and speeds up end-to-end data processing. 

Specially, we implemented two key strategies for reducing storage I/O. First, to minimize redundancy in the mask-based outputs from AI models, we introduced a bitmap-based representation~\cite{ayres2002sequential}. This optimization reduces the original 32-bit output from the AI model to a 2-bit representation, corresponding to a four-class mask, thus reducing the storage footprint to $\frac{1}{16}$ of the original size. Second, once the image reconstruction results are generated, AI segmentation is performed directly in-place within system memory, bypassing the need for storage access and reducing I/O overhead. The only additional storage access occurs when storing the final mask results.
% , as described by the following equation:
% \begin{equation}\footnotesize
% \begin{aligned}
% T_{store_{AI}} &= \sum_{i \in \mathbb{G}} (\lceil \frac{N_z^i}{P_{proj}} \rceil \cdot (\frac{Bitmap(N_x^i \cdot N_y^i)}{P_{vol} \cdot BW_{2ndS}}))
% \label{eq:store-AI}
% \end{aligned}
% \end{equation}
These strategies result in a reduction of more than 40\% in I/O access throughout the entire \emph{ROVAI} workflow, as will be detailed in Section~\ref{sec:evaluation}.


\begin{comment}
\subsection{I/O Optimization Opportunities}
From the hardware perspective, a fundamental limitation emerges when we scale up on the supercomputer, such as Fugaku, adding more nodes increases theoretical computational capability, but the system aggregate I/O bandwidth often remains constrained by physical storage infrastructure.
From the software perspective, image reconstruction and AI-driven segmentation have always been considered as two independent problems. Forcing a workflow where image reconstruction results must be stored as files before the segmentation task begin, requiring repeated retrieval from storage. 
Therefore, the I/O bottleneck is clearly manifested in our problem: as scalability increases, storage I/O constraints inevitably emerge.
The repeated storage access between image reconstruction and AI segmentation becomes a critical performance bottleneck in the ROVAI framework, making it especially important to explore opportunities for reducing storage I/O. We overcome this by two straightforward methods : 1) To minimize the redundancy associated with mask-based outputs from AI models, we employed a bitmap-based representation as an optimization strategy. This directly compresses the original 32-bit AI model output to 2-bit (corresponding to the four-class mask), reducing the storage requirement to $\frac{1}{16}$ of the original size. 2) Once the image reconstruction results are available, AI segmentation is executed directly in-place memory, bypassing storage and reducing I/O overhead. This approach yields a reduction of at least 40\% in I/O access throughout the entire workflow. With these two methods, the only additional storage access introduced during merged AI segmentation is for storing the final mask results.

\begin{equation}\footnotesize
\begin{aligned}
T_{store_{AI}} &= \sum_{i \in \mathbb{G}} (\lceil \frac{N_z^i}{P_{proj}} \rceil \cdot (\frac{Bitmap(N_x^i \cdot N_y^i)}{P_{vol} \cdot BW_{2ndS}}))
\label{eq:store-AI}
\end{aligned}
\end{equation}
\end{comment}




\subsection{Overlapping Imaging \& AI Computations}
The main challenge in fusing image reconstruction with AI segmentation lies in a unified scaling strategy. For model inference, we convert the trained PyTorch model to TorchScript and invoke it from C++ code. This means the model has not been modified for distributed processing. The model can only run on a single node, taking patches after SAP as input and producing same masks of the same dimensions as output.
For image reconstruction, as we discussed in Section~\ref{sec:parallel}, $P_{slice}$ nodes process a single volume slice, and $P_{proj} \times P_{slice}$ nodes process an entire sub-volume. 
To unify the scaling of the two components, we introduce additional communication to ensure that AI segmentation can scale effectively in alignment with the scaling strategy used for image reconstruction. Simultaneously, we minimize the communication overhead to the greatest extent possible.

To that end, as shown in Fig.~\ref{fig:merge_AI}, starting from the distributed image reconstruction results and ending with the distributed mask AI outputs, the distributed process is carried out in five steps: 
1) Distribute SAP method (section \ref{sec:SAP}) on each $P_{slice}$ nodes. Each node retains its own quadtree structure and converts the original volume slice part into continuous patches, 2) Use \emph{MPI\_Alltoallv} communication to transfer only the continuous patches, rather than the raw volume data, across the entire $P_{slice}$ nodes. By this stage, each node has constructed its own complete continuous patches that represent slices of the volume, 3) Perform the (segmentation) model inference on each node, which is equivalent to applying data parallelism over the entire volume across $P_{proj} \times P_{slice}$ nodes, 4) Reverse transfer of the mask patches to their corresponding nodes with \emph{MPI\_Alltoallv} communication, and 5) By using the quadtree structure preserved on each node, the mask patches is transformed to the original volume 2D slice shape. 
% Further updating our performance model,
% These processes can be summarized as $T_{comm_{AI}} + T_{comp_{AI}} + T_{comm_{AI}}$, and are expressed as:
% \begin{equation}\footnotesize
% \begin{aligned}
% T_{comm_{AI}} &= \sum_{i \in \mathbb{G}} (\lceil \frac{N_z^i}{P_{proj}} \rceil \cdot \frac{ N_x^i \cdot N_y^i}{P_{vol} \cdot CC_{other}} + \frac{ V_{SAP}}{TH_{alltoall}^{P_{vol}}})
% \label{eq:comm-AI}
% \end{aligned}
% \end{equation}
% \begin{equation}\footnotesize
% \begin{aligned}
% T_{comp_{AI}} &= \sum_{i \in \mathbb{G}} (\lceil \frac{N_z^i}{P_{proj} \cdot P_{vol}} \rceil \cdot \frac{Model_{AI}}{CC_{AI}})
% \label{eq:comp-AI}
% \end{aligned}
% \end{equation}

So far, we have detailed all stages in \emph{ROVAI}, which are illustrated step by step in Fig.~\ref{fig:pipeline}~(a). 
% \wu{In addition to the times listed in section~\ref{sec:pipeline}, we use $T_{comp}_{AI}$ and $T_{store}_{AI}$ to represent the computational overhead introduced by downstream AI tasks and the overhead associated with PFS storage, respectively.} 
Additionally, we have designed a unified pipeline for \emph{ROVAI}, as shown in Fig.~\ref{fig:pipeline}~(c). AI inference takes considerably longer than image reconstruction, as even though it is optimized by parallel computing, it is more compute intense. Furthermore, as the system scales (e.g. to full Fugaku with 152,064 nodes), the aggregate I/O bandwidth is constrained by the storage sub-system. Our observations indicate that the performance of the entire \emph{ROVAI} framework is ultimately limited by the compute-intense AI inference computation, and PFS I/O operations.

%So far, we have listed all the stages in our \emph{ROVAI} model and we shown each stage step by step in Fig.~\ref{fig:pipeline}a. Furthermore, we designed a unified pipeline for the entire ROVAI framework, as shown in Fig.~\ref{fig:pipeline}c. AI inference takes several times longer than image reconstruction. This is because AI inference, while optimized, does not yield as significant performance as image reconstruction does. In addition, as the nodes scales (such as full Fugaku 152,064 nodes), the system aggregate I/O bandwidth is constrained by physical storage infrastructure. Our observations discovery that the performance of the entire \emph{ROVAI} is finally limited by suboptimal AI inference computation and PFS I/O operations.






==> tex.sc25/9_conclusion.tex <==
\section{Conclusion}
We present \method, a framework that combines high-resolution XCT imaging with AI-driven analytics to improve road infrastructure inspection. Using full Fugaku (152,064 nodes) and SPring-8 imaging, we reconstructed 46 specimens at 8,192 resolution and ran AI segmentation in 2,762 seconds, averaging 60 seconds per specimen. The system reached 60 GB/s I/O bandwidth, utilizing 40\% of the storage capacity. These results show that \method~ can efficiently handle large 3D data and automate defect detection, offering a powerful solution for smarter, data-driven infrastructure management.

